P-MOSS: Scheduling Main-Memory Indexes Over NUMA Servers Using Next Token Prediction

Ever since the Dennard scaling broke down in the early 2000s and the frequency of the CPUs stalled, vendors have started to increase the core count in each CPU chip at the expense of introducing heterogeneity, thus ushering the era of NUMA and Chiplet processors. Since then, the heterogeneity in the design space of hardware has only increased to the point that DBMS performance may vary significantly up to an order of magnitude in modern servers. An important factor that affects performance includes the location of the logical cores where the DBMS queries execute, and the location where the data resides. This paper introduces P-MOSS, a learned spatial scheduling framework that schedules query execution to specific logical cores, and co-locates data on the corresponding NUMA node. For cross-hardware and workload adaptability, P-MOSS leverages core principles from Large Language Models, such as Next Token prediction, Generative Pre-training, and Fine-tuning. In the spirit of hardware-software synergy, P-MOSS guides its scheduling decision solely based on the low-level hardware statistics collected from the hardware Performance Monitoring Unit with the aid of a Decision Transformer. Experimental evaluation is performed in the context of the B$^+$-Tree index. Performance results demonstrate that P-MOSS offers an improvement of up to $6\times$ over traditional schedules in terms of query throughput.

==> sections/Discussion.tex <==
% \section{Discussion}
% yr{What percentile can it eliminate}

==> sections/block.tex <==
\section{Building Blocks of \sys{}}
\label{sec:bb}
Before we move on to the details of \sys, we present an overview of the Performance Monitoring Unit and Offline Reinforcement Learning, i.e., the two respective building blocks of the system and learned component of \sys{}. 

% \subsection{Performance Monitoring Units (PMU)} 
% \label{ss:pmu}
% \noindent\textbf{\blabel{b1}. Performance Monitoring Units (PMU)}
% Modern processors have dedicated hardware blocks throughout the chip, termed Performance Monitoring Unit (PMU, for short), that can track the hardware performance statistics~\cite{pmuIntel,pmuAMD,pmuARM}. These PMUs serve as the building block of \sys{}'s system component. Almost all the hardware components, e.g., the cores, IMCs, interconnects, PCIe lanes of the processor are equipped with their own PMU blocks (cf. Figure~\ref{fig:pmu}). At the core of these PMU blocks, there are multiple counters (1 to 8 depending on the processor and the location of the PMU block) paired with a control register. Also, each PMU provides a fixed list of Performance Monitoring Events. Depending on the location of the PMU (inside or outside a logical core), these events are classified into core and uncore events. Some of the counters are reserved to collect architectural monitoring events, i.e., events that behave consistently across hardware micro-architectures, e.g., the number of executed instructions, 
% % \textcolor{red}{What is retired instruction?}
% % The instructions that enter the processor pipeline and actually gets executed. There might be case when an instruction enters the pipeline but gets flushed right away, if-else if conditions. For clarity I am changing it to executed, but the correct term is retired
% the number of LLC misses, the number of core cycles. The remaining counters can be programmed to monitor a single or multiple (through multiplexing) Performance Monitoring Events through the control registers. 

% % \yr{Have a line that the key principle of sys is to maintain the dbms state through some stuff. Link with goals and say how these components serve them.}



% % \subsection{Offline RL} 
% % \label{ss:offline_rl}
% \noindent\textbf{\blabel{b2}. Offline RL}
% Offline RL serves as the building block of the learned component of \sys{}. In Offline RL~\cite{orl-levine-tut}, the agent is provided with an offline dataset  that consists of various state-action transitions. These transitions represent past experiences collected by running heuristic-based policies under different conditions. In \sys{}, this offline dataset is a collection of \verb|Hardware Snapshots| of the main-memory index. As the system component of \sys{} runs the main-memory index under various scheduling policies for different query workloads and datasets, this dataset can grow overtime. The goal of offline RL is to learn a scheduling policy exclusively from this offline dataset, without any active interaction with the DBMS. 
% % (cf. Figure~\ref{fig:rl_def}). 
% This differs from the traditional RL setting, where the agent learns a new scheduling policy, and then deploys it in the real-world, i.e., into the DBMS for feedback. This can degrade the DBMS performance when the learned policy is sub-optimal. In contrast, there is no feedback loop between the agent and the DBMS in offline RL. The agent is constrained to learn only from the scheduling policies in the provided offline dataset. Hence, during the learning phase, \sys{}'s learned component does not interfere with the DBMS. This presents the opportunity to train \sys{}'s learned agent in a data-driven manner. Despite the difference in technique in how the agent learns a policy in offline RL, the goal of the agent still remains the same, i.e., to maximize a reward function, e.g., query throughput.  
% % This offline dataset provides the opportunity to train \sys{} in a data-driven manner at a larger scale, thereby enabling generalization which is one of the key desired goals of \sys{}. It also poses the opportunity to train the learned component of \sys{} on large neural networks. 

% % yr: I have added these new paragraph as one of reviewers commented about spelling out the challenges of \sys.

\textbf{Why Choose PMU and Offline RL as the Building Blocks of \sys{}?} One of the key challenges of basing \sys{}'s scheduling policy on PMUs alone is that the statistics collected from the PMUs can be non-deterministic, i.e., different runs can generate different values. However, the relative trends in these statistics remain consistent. Also, modern processors provide a large number of hardware events to profile. Hence, it becomes increasingly difficult to hand pick the important hardware statistics that fit across different NUMA architectures, query workloads, datasets, etc. On a similar note, the key challenges of employing offline RL in \sys{} is: How to compile an offline dataset where the state-action transitions can abstract diverse CPU vendors, architectures, query workloads, and data distributions under a generalized framework? This is necessary so that the agent learns to generalize across these different settings. Both PMU and Offline RL work in cohesion to address these challenges. The hardware statistics of PMUs can abstract across these diverse settings to generate high quality data and prepare an offline dataset. In the same manner, the ML techniques employed by the offline RL algorithms are well suited to handle the possible inconsistencies in PMU data as they focus on modeling the wider trends present in the data. Together, they guide the scheduling process in \sys{}. 

% The goal is to learn a policy from this offline dataset by generalizing beyond the collected experiences in the dataset. The agent learns to filter the good experiences, and combine the promising parts of different sub-optimal experiences, and generates a better policy that is not present in the dataset. 
% Lifting the burden of real-time interaction with the environment empowers an offline RL agent to be trained in a data-driven manner with large datasets as well as be equipped with large neural networks. Ironically, the exact same reason makes it challenging for an RL agent to be trained offline. 
% \textcolor{red}{This is all meta talk about offline RL, but you do not say what it is. Use simple language, and there is no need for the meta talk here about the technique before you explain in easy language what the technique that you are proposing is.}
% Since the offline agent cannot interact with the environment, the learned policy can induce states that are missing or hardly present in the static dataset leading to overestimation of the value-estimates, e.g., state-value, action-value functions leading to sub-optimal policies. 
% \textcolor{red}{This last sentence is unclear. Please make it clearer.}
% There exists different bodies of work in the literature to solve offline RL. 
% \textcolor{red}{what do you mean by "solve"? it ORL a problem to be solved or a technique to be used?}
% At the high level, this includes Q-Learning-based 
% \textcolor{red}{Q-learning needs to be defined first. What does Q stand for?}
% approaches that uses Temporal Difference (TD) learning to learn a value function (e.g., ~\cite{KumarZTL20,FujimotoMP19,KostrikovNL22}). 
% \textcolor{red}{The above text looks like a "show-off". Remember that if we lose the reader, we get a reject. We neec to explain what the technique we are using is and not show-off.}
% There also exists imitation-learning-based approaches that mimic the behavioral policy observed in the offline data (e.g., ~\cite{FujimotoG21}). Finally, there is the Transformer-based approach that ditches the traditional 
% \textcolor{red}{TD?}
% TD or imitation-based learning approach and rather treats offline RL as a sequence modeling problem (e.g.,~\cite{ChenLRLGLASM21,ZhengZG22}). 
% \textcolor{red}{all the above does not make much sense here. Is this a literature review? if so, please move to the related work section. Here we need to say what our system does. } 
% The goal 
% \textcolor{red}{goal of what?}
% is to predict a sequence of actions that yield a high sequence of rewards. Refer to~\cite{abs-2203-01387,abs-2005-01643} for a detailed review of various offline RL techniques. 

% After learning an offline policy, one can still
% opt to tune the policy online, with the added benefit that their initial policy is likely safer and cheaper to interact with the environment than an initial random polic
% \begin{figure}[htbp]
%     \centering  \includegraphics[width=0.6\columnwidth]{figures/rl_def.pdf}
%     \caption{Offline vs Online RL.}
%     \label{fig:rl_def}
% \end{figure}
% \textcolor{red}{From this section, we did not learn what p-moss does and how it works or how it uses ORL. Please clarify.}



==> sections/desiderata.tex <==
\section{\sys{}'s Design Considerations}
\label{sec-goals}
We base the design principle of \sys{} on the low-level hardware statistics collected from Performance Monitoring Unit of hardware, and Offline RL to realize the following design objectives.


\noindent\glabel{g1}\textbf%{ Adapting to the Diverse CPU Vendors.} 
{ The Need to Adapt to the Diverse CPU Vendors.} 
In today's hardware landscape, x86 (CISC) and ARM (RISC) are the most prominent processor architectures dominating the computing devices. IBM Power and RISC-v are notable alternatives. Intel and AMD are the leading manufacturers of x86 processors, whereas Apple, Amazon, and NVIDIA use ARM processors in their hardware. Generally, x86 processors have always had the edge over ARM in high performance computing with larger servers. In contrast, ARM processors dominate the smartphone, laptop, and desktop market as they consume less power, and have a reduced instruction set architecture.  
% \textcolor{red}{Previous sentence needs a fix. It does not read right.}
In recent times, ARM processors have become increasingly popular in servers, which begs the need for rethinking DBMS components for the ARM processors. 
%as well. 
Processors with the same architecture but from different vendors also exhibit distinct characteristics, e.g., Intel Skylake X distributes the L3 cache into slices across all the cores, whereas in AMD EPYC Rome, all cores in a Core Complex Die share a unified L3 cache. The same applies for the ARM processors built by different CPU vendors. Hence, a key goal of \sys{} is to maintain robust behavior across diverse vendors, while adapting to its unique characteristics for optimal performance.
% Thus, taking the unique characteristic of the diverse cpu architecture and vendors into account is an important design choice. 
% \textcolor{red}{The previous section does talk about the diversity in architectures but does not talk about the "adapting" part that is in Goal 1 title. Also, the title "Adapting to the Diverse CPU vendors" is not specific and can elude to be similar to the sentence of Goal 2. May be we need to make it more specific, e.g., Adapting to the Diversity in Instruction Sets, or something along this line that is more specific.}


\noindent\glabel{g2}\textbf%{ Adapting to the ever evolving landscape of NUMA architecture.} 
{ The Need to Adapt to the Ever Evolving Landscape of NUMA Architectures.} 
The landscape of NUMA architectures is always evolving, e.g., in earlier multi-socket NUMA servers,
%such as 
e.g.,
Intel Sandy Bridge, there is no localization within a socket, i.e., each NUMA socket has one NUMA node and one Integrated Memory Controller (IMC). This introduces excessive traffic on the memory channels for processors with high core count. To relieve the 
%pressure 
contention 
on the memory channels, later versions introduce more than one IMC in a single NUMA socket (e.g., Intel Ice Lake), and logically divide the cores, caches, and memory controllers into multiple NUMA nodes (e.g., Intel Skylake X). This introduces non-uniformity in the memory access latency even within a socket. The latest chiplet-based NUMA architectures, e.g., AMD EPYC Rome and Intel Sapphire Rapids, has further expanded this idea by physically assembling multiple chips inside a NUMA socket, and hence broadening the range of non-uniformity within a NUMA socket. 
AMD EPYC Milan and Rome have 
%gone further and ditched the
abandoned the use of IMCs in favor of a unified memory controller on a different chip. Hence, a key goal for \sys{} is to adapt to these diverse NUMA architectures.
% \textcolor{red}{Again, this section talks to the diversity in NUMA architectures but does not talk to the Goal statement, which is the need to adapt.}
\vspace{-3mm}
\begin{figure}[htbp]
    \captionsetup{belowskip=-8pt}
    \captionsetup{aboveskip=-1pt}
    \centering
    \includegraphics[width=\columnwidth]{figures/numa_machine1.pdf}
    \caption{The socket layout of various NUMA %architecture.}
    architectures.}
    \label{fig:numa_eval}
\end{figure}

\noindent\glabel{g3}\textbf%{ Handling Heterogeneous Query Workloads.} 
{ The Need to Handle Heterogeneous Query Workloads.}
DBMS workloads are diverse, e.g., OLTP vs. OLAP at the applications level. Similarly, at the \textit{hardware level}, workloads vary greatly in terms of their compute vs. memory accesses. The number of data requests generated by a lookup query served by a main-memory index is very small compared to a range scan, where the number of data requests can be very large depending on selectivity. Depending on the size of the result generated by a lookup or a range scan, different queries also exhibit different compute characteristics. A query executes a lower number of CPU instructions when the generated result size is small compared to when the result size is large. On top of that, query workloads are dynamic and can change frequently. 
For example, in scientific databases, the focus shifts from one data space to another on a daily basis for exploratory data analysis as new data is received periodically~\cite{GraefeIKM10}. In such cases, the optimization needs to be swift and immediate. Thus, a key design decision for \sys{} is whether to treat the diverse characteristics of the query workloads differently, and if so, how, while being swift. 

% \textcolor{red}{Add the word PMOSS in the above sentence. Also, you need to add a similar conclusion sentence to each of the other two goals above.}

% \noindent\glabel{g4}\textbf{ Handling Dynamic Exploratory Query Workloads.} Query workloads can be dynamic and change frequently. For example, restaurants in a downtown area tend to be more crowded during weekends than weekdays. Depending on the span of a query workload, the workload can also shift on an hourly, daily, or weekly bases. For example, the trending topic on Twitter changes on hourly basis. In scientific databases, the focus shifts from one data space to another on a daily or weekly basis for exploratory data analysis as new data is received 
% periodically~\cite{GraefeIKM10}. In such cases, where the workload shifts rapidly, the optimization needs to be swift and immediate as well. 
% \textcolor{red}{I suggest merging goals 1 and 2 together, and 3 and 4 together, as they are close.}

\noindent\glabel{g4}\textbf{ The Need to Handle Conflicts. } 
For optimal performance, the synergy between the %DMBS, and the OS as well the hardware is a must. 
DMBS, the OS, and the underlying hardware is necessary. 
However, there might be fundamental conflicts among their objectives. For example, the objective of the IMC is to ensure a higher DRAM throughput. Hence, it prioritizes sequential memory requests over random ones in its queue~\cite{DasAMKA13}. 
This contrasts with the objective of the DBMS, i.e., to ensure a higher query throughput. For DBMSs, prioritizing sequential memory requests over random ones will result in \textit{interference} among concurrently running queries leading to a lower query throughput. For example, a lookup query may delay or starve due to a surge of concurrently running range scans. 
% \textcolor{red}{Does IMC prioritize this way to help the DBMS or to help itself? You may need to move this previous sentence up a bit before you talk about the objectives of the DBMS to avoid the confusion.}
% One of the negative side-effects that stems from this conflict 
Similarly, the objective of the OS slab allocator is to allocate the least amount of memory space by reducing the memory defragmentation, not accounting for the data hotness. This may lead to both hot and cold data being packed together in the same memory page, and hence leading to sub-optimal performance, e.g., high TLB (Translation Lookaside Buffer) misses~\cite{StoicaA13,WongFXLK15}. Hence, a key objective for \sys{} is to keeping these conflicts between the DBMS, the OS and the hardware to a minimum.
% higher DTLB misses. 
% \textcolor{red}{what is DTLB? let alone its misses. to avoid having to explain this, use higher level language, and then say: e.g., high DTLB misses and give a reference.}


\noindent \glabel{g5}\textbf{ 
% Tight Coupling of Machine Learning in DBMSs with Minimum Overhead.
The Need to Isolate the Learning Process from DBMSs in ML4DB Systems}. Reinforcement Learning (RL) has emerged as one of the more popular Machine Learning (ML) techniques in Machine Learning for Database (ML4DB) systems for building learned components, e.g., table partitioners~\cite{HilprechtBR20}, job schedulers~\cite{MaoSVMA19,SabekUK22}, knob tuners~\cite{ZhangLZLXCXWCLR19,LiZLG19}, join order selector~\cite{OrtizBGK18,abs-1808-03196}, 
and query optimizer~\cite{MarcusNMZAKPT19,MarcusNMTAK21}. These learned components fundamentally follow the \textit{online} learning paradigm, termed Online RL, that requires the agent to actively interact with the DBMS, and collect experience based on the latest learned policy to improve upon itself. What distinguishes RL from other ML techniques is the concept of \textit{exploration-exploitation},
%which means that
i.e., 
the agent has to go through a continuous process of making mistakes, and progressively learning from these mistakes
until it reaches a stable state. In the context of Online RL, this involves the agent taking sub-optimal decisions (actions) over a long period that may degrade the DBMS performance in an unpredictable manner. The exact same reason makes Online RL impractical for dynamic exploratory query workloads, 
especially 
when the span of the query workload is comparatively short. By the time an agent is optimized for a certain query workload, the workload has already changed, leaving the agent trapped in a never ending cycle of playing catch-up. Hence, it's of utmost importance that \sys{} decouples the learning process from the DBMS operations. 
% \textcolor{red}{Is the goal "to avoid tight coupling" or "to have tight coupling"? The goal title is confusing. Add always a concluding sentence per goal to say how this relates or should relate to PMOSS.}







% \yr{Discuss how great PMU can be, this section needs to be looked over again.}
% \todo{Pitfalls of Sampling: Discuss, this introduces additional compute overhead that's got nothing to do with query execution. This also pollutes the cache (we also do it though)}
% \yr{The key to the success of ML can be boiled down to data distribution. How existing ML4DB does this and we introduce the hardware counters as the way to go. And why using hardware counters can be the way to go}



